Dynamic Objective MPC for Motion Planning of Seamless Docking Maneuvers

Automated vehicles and logistics robots must often position themselves in narrow environments with high precision in front of a specific target, such as a package or their charging station. Often, these docking scenarios are solved in two steps: path following and rough positioning followed by a high-precision motion planning algorithm. This can generate suboptimal trajectories caused by bad positioning in the first phase and, therefore, prolong the time it takes to reach the goal. In this work, we propose a unified approach, which is based on a Model Predictive Control (MPC) that unifies the advantages of Model Predictive Contouring Control (MPCC) with a Cartesian MPC to reach a specific goal pose. The paper's main contributions are the adaption of the dynamic weight allocation method to reach path ends and goal poses inside driving corridors, and the development of the so-called dynamic objective MPC. The latter is an improvement of the dynamic weight allocation method, which can inherently switch state-dependent from an MPCC to a Cartesian MPC to solve the path-following problem and the high-precision positioning tasks independently of the location of the goal pose seamlessly by one algorithm. This leads to foresighted, feasible, and safe motion plans, which can decrease the mission time and result in smoother trajectories.

==> plots/evaluation/carla_test/carla_test.tex <==
% \tikzset{external/export next=false}

% Trajectories
\pgfplotstableread[col sep=comma,]{plots/evaluation/carla_test/cleaned_carla_test_driven.csv}\driventable

% Corridor and goal
\pgfplotstableread[col sep=comma,]{plots/evaluation/carla_test/cleaned_carla_test_corridor.csv}\corridortable
\pgfplotstableread[col sep=comma,]{plots/evaluation/carla_test/cleaned_carla_test_goal_pose.csv}\goaltable


\begin{tikzpicture}
    \begin{axis}[
        width=0.9\linewidth,
        height=6cm,
        axis equal,
        clip marker paths=true,
        ylabel=y in $m$,
        xlabel=x in $m$,
        % xmin=-5.5,
        % xmax=20,
        % ymin=-26,
        % ymax=1,
        legend columns = 4,
        legend style={at={(1.0, 1.02)},anchor=south east, /tikz/every even column/.append style={column sep=0.1cm}},
    ]

    \addplot[
        color=black, 
        line width=1pt,
        color=black,
        each nth point=2,
    ] 
    table [
        x=x_bound_left, 
        y=y_bound_left, 
    ] {\corridortable};
    \addlegendentry{corridor}
    
    \addplot[
        color=black, 
        line width=1pt,
        color=black, 
        each nth point=2,
        forget plot
    ] 
    table [
        x=x_bound_right, 
        y=y_bound_right, 
    ] {\corridortable};

    \addplot[
        color = matlabBlue,
        only marks,
        mark=*, 
        mark size=0.4mm,
    ] 
    table [
        x=sim_x, 
        y=sim_y,
    ] {\driventable};
    \addlegendentry{ours}

    \addplot[
        color=newGray, 
        line width=1pt,
        each nth point=2,
    ] 
    table [
        x=path_x, 
        y=path_y, 
    ] {\corridortable};
    \addlegendentry{path}
    
    % Ego vehicle
    \addplot[
        line width=1pt,
        color=matlabDarkRed
    ] 
    table [x=x, y=y] {\goaltable};
    \addlegendentry{goal pose}
    
    \addplot[
        line width=1.5pt,
        color=matlabDarkRed
    ] 
    table [x=rl_x, y=rl_y] {\goaltable};
    \addplot[
        line width=1.5pt,
        color=matlabDarkRed
    ] 
    table [x=rr_x, y=rr_y] {\goaltable};
    \addplot[
        line width=1.5pt,
        color=matlabDarkRed
    ] 
    table [x=fl_x, y=fl_y] {\goaltable};
    \addplot[
        line width=1.5pt,
        color=matlabDarkRed
    ] 
    table [x=fr_x, y=fr_y] {\goaltable};
    
    \end{axis}
\end{tikzpicture}


